Learning Neuro-Symbolic Relational Transition Models for Bilevel Planning

In robotic domains, learning and planning are complicated by continuous state spaces, continuous action spaces, and long task horizons. In this work, we address these challenges with Neuro-Symbolic Relational Transition Models (NSRTs), a novel class of models that are data-efficient to learn, compatible with powerful robotic planning methods, and generalizable over objects. NSRTs have both symbolic and neural components, enabling a bilevel planning scheme where symbolic AI planning in an outer loop guides continuous planning with neural models in an inner loop. Experiments in four robotic planning domains show that NSRTs can be learned after only tens or hundreds of training episodes, and then used for fast planning in new tasks that require up to 60 actions and involve many more objects than were seen during training. Video: https://tinyurl.com/chitnis-nsrts

==> ablation_stds_table.tex <==
\begin{table*}[ht!]
	\centering
	\footnotesize
	\begin{tabular}{| l | p{0.68cm} | p{0.68cm} | p{0.68cm} | p{0.68cm} | p{0.68cm} | p{0.68cm} | p{0.68cm} | p{0.68cm} | }
	\hline
	\multicolumn{1}{|c|}{} &\multicolumn{2}{c|}{PickPlace1D} &
	\multicolumn{2}{c|}{Kitchen} &
	\multicolumn{2}{c|}{Blocks} &
	\multicolumn{2}{c|}{Painting} \\
	\hline
	\emph{Methods} &
	{\scriptsize Easy} & {\scriptsize Hard} &
	{\scriptsize Easy} & {\scriptsize Hard} &
	{\scriptsize Easy} & {\scriptsize Hard} &
	{\scriptsize Easy} & {\scriptsize Hard} \\
	\hline
    Bilevel planning with NSRTs (Ours) & 2.826 & 15.492 & 0.599 & 2.736 & 1.414 & 3.935 & 0.696 & 8.731 \\
    Bilevel planning with prior (B6) & 3.140 & 8.425 & 9.778 & 10.295 & 5.510 & 10.735 & 15.882 & 0.331 \\
    Forward shooting with prior (B7) & 4.106 & 0.000 & 0.000 & 1.323 & 4.807 & 2.736 & 3.276 & 0.000 \\
    \hline
	\end{tabular}
	 \caption{This table, referenced in \appref{subsec:ablationstds}, is a companion to Table \ref{tab:ablations} in the main text, showing the numerical standard deviations of the means. See Table \ref{tab:ablations} caption in \secref{sec:experiments} for details.}
	\label{tab:ablationstds}
\end{table*}

